Inter-regional correlation estimators for functional magnetic resonance imaging

Functional magnetic resonance imaging (fMRI) functional connectivity between brain regions is often computed using parcellations defined by functional or structural atlases. Typically, some kind of voxel averaging is performed to obtain a single temporal correlation estimate per region pair. However, several estimators can be defined for this task, with various assumptions and degrees of robustness to local noise, global noise, and region size. In this paper, we systematically present and study the properties of 9 different functional connectivity estimators taking into account the spatial structure of fMRI data, based on a simple fMRI data spatial model. These include 3 existing estimators and 6 novel estimators. We demonstrate the empirical properties of the estimators using synthetic, animal, and human data, in terms of graph structure, repeatability and reproducibility, discriminability, dependence on region size, as well as local and global noise robustness. We prove analytically the link between regional intra-correlation and inter-region correlation, and show that the choice of estimator has a strong influence on inter-correlation values.

==> supplementary_materials.tex <==
\section{Proposition and proof for estimator D}
\label{sup:s:prop_proof_D}.
	\jf{More formally, we have the following result which helps in establishing~\eqref{eq:D}.
		
		\begin{prop}\label{prop:disconnected} Under the notation of this section, as $T \to \infty$, the following statements hold almost surely. \\
			(i) 
			\begin{equation*}
				\widehat \cov ( \Vect{Y}_{i^{(b)}} - \Vect{Y}_{k^{(b)}} , \Vect{Y}_{i^{\prime(b)}} - \Vect{Y}_{k^{\prime(b)}}) \stackrel{a.s.}{\to} \sigma_j \sigma_{j^\prime} r_{jj^\prime}.
			\end{equation*}
			(ii)
			\begin{equation}
				2 \widehat{s}^2(\Vect{Y}_{i^{(b)}} ,\Vect{Y}_{k^{(b)}} , \Vect{Y}_{k^{\prime(b)}} ) \stackrel{a.s.}{\to} 2\sigma_j^2 + 2 \sigma_\varepsilon^2.
			\end{equation}
		\end{prop}
		
		
		\begin{proof}
			(i) Using the independence in time, it is clear that the left-hand side converges almost surely to $\cov ( {Y}_{i^{(b)}}(1) - {Y}_{k^{(b)}}(1) , {Y}_{i^{\prime(b)}}(1) - {Y}_{k^{\prime(b)}}(1)) = \sigma_j \sigma_{j^\prime} r_{jj^\prime}+ \sigma_e^2 - 2 \sigma_e^2 + \sigma_e^2$ since the two regions $\r_k$ and $\r_{k^\prime}$ are disconnected,  which leads to the result. \\
			(ii) In the same way, the left-hand side tends to $\var(Y_{i^{(b)}}(1) - {Y}_{k^{(b)}}(1)) + \var(Y_{i^{(b)}}(1) - {Y}_{k^{\prime(b)}}(1)) - \var(Y_{k^{(b)}}(1) - {Y}_{k^{\prime(b)}}(1)) = \sigma_j^2 + \sigma^2_k+\sigma_{k^\prime}^2 + 4 \sigma_\varepsilon^2 - \sigma_k^2-\sigma^2_{k^\prime} - 2\sigma_\varepsilon^2$ which yields the stated limit.
		\end{proof}
		
		In other words, Proposition~\ref{prop:disconnected} shows that $\widehat{r}^\D_{jj^\prime}$ is a strongly consistent estimator of $r^\D_{jj^\prime}$ given by
		\begin{equation}
			r^\D = r_{jj^\prime} \; \; \frac{1 }{
				\sqrt{	\left( 1 +  \sigma_{\varepsilon,j}^2 \right) 
					\left( 1 +  \sigma_{\varepsilon,j^\prime}^2 \right) }
			}
			\label{eq:D}
		\end{equation}
		which, in the situation where $\sigma_\varepsilon=0$, is nothing else than $r_{jj^\prime}$.

